DecoFuse: Decomposing and Fusing the "What", "Where", and "How" for Brain-Inspired fMRI-to-Video Decoding

Decoding visual experiences from brain activity is a significant challenge. Existing fMRI-to-video methods often focus on semantic content while overlooking spatial and motion information. However, these aspects are all essential and are processed through distinct pathways in the brain. Motivated by this, we propose DecoFuse, a novel brain-inspired framework for decoding videos from fMRI signals. It first decomposes the video into three components - semantic, spatial, and motion - then decodes each component separately before fusing them to reconstruct the video. This approach not only simplifies the complex task of video decoding by decomposing it into manageable sub-tasks, but also establishes a clearer connection between learned representations and their biological counterpart, as supported by ablation studies. Further, our experiments show significant improvements over previous state-of-the-art methods, achieving 82.4% accuracy for semantic classification, 70.6% accuracy in spatial consistency, a 0.212 cosine similarity for motion prediction, and 21.9% 50-way accuracy for video generation. Additionally, neural encoding analyses for semantic and spatial information align with the two-streams hypothesis, further validating the distinct roles of the ventral and dorsal pathways. Overall, DecoFuse provides a strong and biologically plausible framework for fMRI-to-video decoding. Project page: https://chongjg.github.io/DecoFuse/.

==> tables/IoU-result.tex <==
\begin{table}[]
	\begin{tabular}{ccl}
		\toprule
		Methods        & IoU(background)      & IoU(foreground)           \\ \hline
		fMRI-PTE-video & \multicolumn{1}{l}{} &                           \\
		w/o where      &                      &                           \\
		w/i where      & 0.656                & \multicolumn{1}{c}{0.219} \\ \bottomrule
	\end{tabular}
	\caption{IoU results}
\end{table}

==> tables/motion-result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htbp]
	\begin{tabular}{cccc}
		\toprule
		& Methods & cosine similarity & end point error \\ \hline
		\multirow{2}{*}{subject 1} & CMU     & 0.174             & 1.72            \\
		&         & 0.138             &                 \\ \hline
		\multirow{2}{*}{subject 2} & CMU     & 0.085             & 1.72            \\
		&         &                   & \textbf{}       \\ \hline
		\multirow{2}{*}{subject 3} & CMU     & 0.110             & 1.76            \\
		&         & \textbf{}         & \textbf{}       \\ \bottomrule
	\end{tabular}
\caption{motion prediction results.}
\end{table}


% valid ratio > 0% -> 10% .... 60%

%# sub1:
%#     0.1262039691209793
%#     0.13855904340744019
%#     0.1385076344013214
%#     0.14707264304161072
%#     0.15016306936740875
%#     0.21221843361854553
%#     0.17925722897052765
%# sub2:
%#     0.03960904851555824
%#     0.04424474760890007
%#     0.04516442492604256
%#     0.05170568451285362
%#     0.05547219142317772
%#     -0.027964303269982338
%#     -0.1369106024503708
%# sub3:
%#     0.07729573547840118
%#     0.08809065073728561
%#     0.10632021725177765
%#     0.12854693830013275
%#     0.1533174216747284
%#     0.1441621333360672
%#     0.049786075949668884
